Neuromorphic Programming: Emerging Directions for Brain-Inspired Hardware

The value of brain-inspired neuromorphic computers critically depends on our ability to program them for relevant tasks. Currently, neuromorphic hardware often relies on machine learning methods adapted from deep learning. However, neuromorphic computers have potential far beyond deep learning if we can only harness their energy efficiency and full computational power. Neuromorphic programming will necessarily be different from conventional programming, requiring a paradigm shift in how we think about programming. This paper presents a conceptual analysis of programming within the context of neuromorphic computing, challenging conventional paradigms and proposing a framework that aligns more closely with the physical intricacies of these systems. Our analysis revolves around five characteristics that are fundamental to neuromorphic programming and provides a basis for comparison to contemporary programming methods and languages. By studying past approaches, we contribute a framework that advocates for underutilized techniques and calls for richer abstractions to effectively instrument the new hardware class.

==> old/nmp-may2.tex <==

\label{s:neuromorphic-programming}
%DC has had decades to build abstraction and compilation hierarchies to facilitate the programming of increasingly complex computer systems.

INTRODUCTION

Requirements for NMP:
- robustness
- abstractions
- etc.

% % others: continual operation, information/knowledge representation

% \paragraph{Robustness} Any computational system must have some \emph{robustness} against external influences. In digital computers, this stems from the strong dynamical robustness of bi-stable switching dynamics. Thus, the physics of digital computing is very robust, but the computation itself is brittle---a single bit flip can lead to catastrophic failure. 
% In contrast, the brain works reliably despite noise, neuron death, and re-generation. Natural systems like the brain use robust adaptive procedures on a computational level \cite{SimonLaird2019}.

% \paragraph{Abstraction} A central tool of computer science is \emph{abstraction}, which allows programmers to manage complexity by layering different levels of system functionality. This multi-scale organization mirrors the hierarchical structures found in biological brains, where complex networks operate on various temporal and spatial scales to process information efficiently. 
% Abstractions in digital computing yield decomposable hierarchies \cite{Simon1991,Booch2011}. The brain also shows a hierarchical organization, albeit with more intricate interactions that do not lend themselves to a clean decomposition, instead leading to \emph{nearly} decomposable hierarchies \cite{Simon1991}.
% We presently lack mathematical tools to capture complex interactions of nonlinear phenomena at different spatio-temporal scales, and we lack programming methods to harness dynamics on multiple timescales. 
% This is also evident in Figure \ref{fig:hero} that plots the \textit{domain} and \textit{plasticity} axes of a select number of programming technologies.
% To the knowledge of the authors, no programming abstractions have been developed that capture the plasticity of the computational substrate while operating on digital and analog signals alike.

%Schuman: backprop, conversion, reservoir, evolution, plasticity
%Further: non-ML algs, programming abstractions

%Offline off-device optimization methods are most mature as they have been advanced by computer science and machine learning for decades. 
%
%Off-chip online optimization methods also benefit from extensive work done in the fields of computer science, machine learning, and signal processing.
%{\color{red}TODO give examples}.
%
%{\color{red}TODO rewrite}
%
%Some offline optimization methods can be implemented directly on-device, such as equilibrium propagation \cite{KendallEtAl2020Training}, and efforts exist to implement gradient-based methods on-device as well \cite{BoonEtAl2021Gradient}.
%
%Off-chip online optimization methods also benefit from extensive work done in the fields of computer science, machine learning, and signal processing. {\color{red}TODO give examples}.
%These methods can also be adapted to the on-device setting, although this is often difficult in practice because the computations required to implement these optimization methods are often costly in terms of area and energy on device. For this reason, self-organization methods are a popular alternative for online on-device learning. 
%In an on-device, online settings, optimization methods from the off-device, online setting can be implemented. 

\paragraph{Neuromorphic co-design}
% manual design -> starting point
% gives an upper bound for the flexibility one can have
As neuromorphic computers exploit physical phenomena of their underlying hardware, manually designed neuromorphic programs will necessarily be close to physics. Therefore, although not strictly a `programming' paradigm, it is instructive to consider \textbf{neuromorphic co-design} as a paradigm for designing neuromorphic systems.
The field is rooted in the original vision of neuromorphic computing \cite{Mead1990} and designs application-specific and reconfigurable mixed-signal neuromorphic chips in sub-threshold CMOS technology. 
This approach uses tools from signal processing and computational neuroscience to implement a desired behavior in networks of silicon neurons \cite{IndiveriEtAl2011}. 
Similar to analog computing, the field may benefit from a set of computational primitives to simplify the design of neuromorphic systems.

\paragraph{Machine learning methods}
Given the success of deep learning, learning is a natural paradigm for neuromorphic computers. 
While it would be naïve to ignore the deep learning literature, it is also unrealistic to expect deep learning methods to work for SNNs as well as they do for ANNs since these methods were optimized for ANNs \cite{DaviesEtAl2021Advancing}. 
%
% To compile a neural network into hardware, it is necessary to first design the neural network's architecture. Deep learning has accumulated a plethora of well-performing network architectures for ANNs 
\emph{ANN-to-SNN conversion} is possible but typically not optimal because the resulting SNN typically does not leverage the computational power of spiking neurons and instead limits the richer dynamics of SNNs to the same less powerful domain of ANNs \cite{SchumanEtAl2022Opportunities}.
%
\emph{Backpropagation}, the workhorse of deep learning, can be implemented directly in SNNs using surrogate gradients \cite{Eshraghian2023training} or other neuromorphic adaptations. 
% Simplifications of the backpropagation algorithm such as the random backpropagation algorithm \cite{BaldiEtAl2018Learning} were also demonstrated in neuromorphic systems \cite{NeftciEtAl2017}. 
It is also possible to create a \emph{surrogate model} of the physical device, then optimize the surrogate model in simulation with deep learning methods and transfer the optimized model back to the device \cite{EulerEtAl2020deep,HeEtAl2019}.
%
% 
Given a neural network, it is necessary to communicate this network to the hardware. 
\emph{Neuromorphic compilation} \cite{ZhangEtAl2020} was proposed as a general framework to (approximately) compile neural networks into different hardware systems, automatically adapting to physical constraints. 
% Such compilation can be done statically to exactly implement the specified network architecture \cite{GruauEtAl1995neural,Siegelmann1994Neural}, or adaptively to further optimize the network after compilation \cite{BunelEtAl2016Adaptive}. In any case, it is important to consider the hardware constraints in this compilation \cite{JiEtAl2018Bridge}.
%
Compilation and conversion are promising directions, though descriptions at the level of neural network architectures may not provide a high enough abstraction for implementing programs that realize arbitrary computations. 

For recurrent neural networks, \emph{reservoir computing} avoids the need to backpropagate information through the network to compute gradients. Instead, the reservoir is kept fixed and only a readout map from the reservoir to the output is trained. This training procedure requires the reservoir states to be read out and stored, which may not be possible given limited observability of some devices or limited data storage. Reservoir computing is a popular paradigm for neuromorphic computing, with dedicated frameworks for hardware implementation \cite{SchumanEtAl2022Opportunities,Michaelis2020}.

\paragraph{Online learning}
The machine learning methods presented above all operate offline and often off-device. Frequent re-training creates a large overhead, limiting the performance and applicability of neuromorphic computers. 
%
As a result, \emph{on-device learning} methods are an active topic of research \cite{BasuEtAl2018Low}. 
\emph{Plasticity} is a popular paradigm for on-device learning where local learning rules are used to modify the connectivity (structural plasticity) and connection strengths (synaptic plasticity) of a SNN.
Parallels to emergent programming may be drawn here as the resulting behavior of the SNN emerges from the interaction of local rules. It is not clear what local rules will yield a particular network-level behavior, but evolutionary search \cite{JordanEtAl2020} and meta-learning \cite{ConfavreuxEtAl2020} have been used to (re-)discover desirable plasticity rules.

\paragraph{Evolutionary methods}
A key advantage of evolutionary approaches is that they can jointly optimize the network's architecture and weights, thus simultaneously designing and training the network. Moreover, evolutionary methods do not require differentiability of activation functions, nor do they place any constraints on the network's architecture. 
Evolutionary approaches can find a SNN by randomly choosing an initial population of candidate SNNs, selecting the highest-performing candidates according to some performance metric, and then creating new candidates through recombining and mutating the selected candidates \cite{SchumanEtAl2020Evolutionary,SchliebsKasabov2013Evolving}. 
However, evolutionary approaches can be slower to converge than other training methods \cite{SchumanEtAl2022Opportunities} and the resulting architectures are not easily interpretable or reusable for different tasks \cite{Conrad1988}.

\paragraph{Spiking neuromorphic algorithms}
With the increased availability of neuromorphic hardware, a number of handcrafted spiking neuromorphic algorithms (SNA) have been proposed. SNAs implement computations using temporal information processing with spikes, often to implement well-defined computations such as functions on sets of numbers \cite{VerziEtAl2018Computing}, functions on graphs \cite{HamiltonEtAl2019Spike}, solving constraint satisfaction problems or solving a steady-state partial differential equation using random walks \cite{SmithEtAl2020Solving}.
SNAs are being actively developed and many application domains are yet to be explored \cite{Aimone2019}.
% A number of handcrafted SNN algorithms have been proposed in recent years to solve well-deﬁned computational problems using spike-based temporal information processing. When implemented on neuromorphic architectures, these algorithms promise speed and efﬁciency gains by exploiting ﬁne-grain parallelism and event-based computation. Examples include computational primitives, such as sorting, max, min, and median operations [70], a wide range of graph algorithms [71]–[74], NP-complete/hard problems, such as constraint satisfaction [75], boolean satisﬁability [76], dynamic programming [77], and quadratic unconstrained binary optimization [78], [79], and novel Turing-complete computational frameworks, such as Stick [80] and SN P [81].

% primitives and synthesis
\paragraph{Neurocomputational primitives}
A variety of neurocomputational primitives have been proposed in the neuromorphic community. Such primitives can be useful for simple tasks and typically allow for composability to create more complex neuromorphic systems at a higher level of abstraction \cite{BartolozziEtAl2022Embodied,MarcusEtAl2014}.
% WTA & DNF
\textbf{Dynamic neural fields} (DNFs) are a modern framework for neural attractor networks \cite{Giese_1999, Schoener2019}. The stable states provided by attractor dynamics help with the intrinsic variability of analog neuromorphic circuits and have been shown to be a promising abstraction for neuromorphic programming \cite{DaviesEtAl2021Advancing}.
Each DNF is a network of neurons that is, under some constraints, computationally equivalent to a \textbf{winner-take-all} (WTA) network \cite{Sandamirskaya2014Dynamic}. The WTA is a common circuit motive in the neocortex \cite{DouglasMartin2007Recurrent}.
%Computation with attractor networks has a rich history in neural computation \cite{Hopfield1982} and provides a simple way for ....... neurosymbolic integration.
% NSM
The \textbf{neural state machine} (NSM) \cite{NeftciEtAl2013,LiangEtAl2019Neural} also builds on WTA networks to implement finite state machines in SNNs, and has been shown to run robustly on mixed-signal neuromorphic hardware.
% sPLL
The \textbf{spiking phase-locked loop} (sPLL) \cite{MastellaChicca2021} was designed for frequency detection as part of a neuromorphic tactile sensor.
% TDE
The \textbf{temporal difference encoder} (TDE) \cite{MildeEtAl2018,GutierrezGalanEtAl2021Event} is a spiking model that was designed to compute the time difference between two consecutive input spikes. The number of output spikes and the time between them is inversely proportional to the time difference. This has been used for motion estimation and obstacle avoidance \cite{MildeEtAl2017Obstacle}.
%Delay/Temporal measurement circuits take inspiration from the insect brain, where motion is computed as the time to travel of a stimulus from one sensing element to the neighbour 180 . This type of computational primitive is useful for motion estimation and obstacle avoidance 88 
% for temporal encoding on event-based signals, which translates the time difference between two consecutive input events into a burst of output events. The number of output events along with the time between them encodes the temporal information.
%The TDE unit translates the time difference between two events into a burst of output spikes. Both the number of output spikes and the duration of the burst produced by the model directly reflect the temporal correlation of two input signals, and it is inversely proportional to the time difference
\textbf{Neural oscillators} generate rhythmic activity that can be used for feature binding and motor coordination, for example as a central pattern generator \cite{KrauseEtAl2021Robust}.
% Further
Other primitives are scattered around the literature and shared libraries of neurocomputational primitives are only starting to be assembled \cite{BartolozziEtAl2022Embodied}.
%
\textbf{Neuromorphic synthesis} \cite{NeftciEtAl2013} may provide a systematic way of programming complex high-level behavior into neuromorphic chips. This was demonstrated for functions that can be described by finite state machines, but it may be promising to extend this work to a larger set of computational primitives for higher abstractions in neuromorphic programming.

\paragraph{Higher abstractions}
% NEF
The \emph{neural engineering framework} \cite{EliasmithAnderson2002Neural} raises the level of abstraction beyond the level of neural networks. This allows dynamical systems to be distilled automatically into networks of spiking neurons that can then be compiled down to mixed-signal spiking neuromorphic accelerators like Braindrop \cite{NeckarEtAl2019} using the Nengo programming environment \cite{BekolayEtAl2014}.

% VSA
The \emph{vector symbolic architectures} (VSA) framework is suitable for neuromorphic systems, enabling knowledge representation and reasoning in high-dimensional spaces.
% Vector symbolic architectures (VSAs) offer a mathematical, connectionist framework that supports rich knowledge representations and reasoning in high-dimensional spaces. 
VSAs interfaced with deep networks and generalizations of the optimization and search algorithms described in this survey could provide a path to enabling fast, efficient, and scalable next-generation AI capabilities on neuromorphic hardware.

% Lava
Intel recently launched \emph{Lava}\footnote{\href{https://github.com/lava-nc/lava}{github.com/lava-nc/lava}}, an open-source neuromorphic programming framework for the Loihi chips. Support for other neuromorphic hardware is planned. Lava is a multi-paradigm framework and includes libraries of neuromorphic algorithms for optimization, attractor networks, deep learning methods for SNNs, VSAs, and plans to include more paradigms.

% Fugu
Aimone \textit{et al.} \cite{AimoneEtAl2019Composing} proposed \emph{Fugu}, a hardware-independent mechanism for composing different SNAs. In Fugu, a program is specified as a computational graph reminiscent of dataflow programming, where nodes represent SNAs and connections represent dataflow between the SNAs. 
%Each SNA has a certain input size and output size (number of inputs and time length) in addition to a circuit depth which specifies how many timesteps are necessary for incoming data to be processed. The entire program is specified by the neural circuit that includes all SNAs and their interconnections. 
This program can then be compiled into different hardware-specific configurations. The focus of this work is on digital neuromorphic processors and support for mixed-signal hardware is not discussed.
%Fugu: hardware-independent mechanism for linking a variety of scalable spiking neural algorithms from a variety of sources. Individual kernels linked together provide sophisticated processing through compositionality. \cite{AimoneEtAl2019Composing}

\paragraph{Others}
\textbf{Emergent programming} uses multiple interacting sub-programs whose collective behavior constitutes the desired program. The individual instructions are typically not explicitly informed of the program to be created \cite{GeorgeEtAl2005Experiments}. 
% This approach has been used to design programs that exhibit some creativity \cite{Hofstadter1991}. This is reminiscent of local learning rules in neuromorphic computers (see Section \ref{ss:neuromorphic-programming}).
%, by using methods from adaptive multi-agent systems and relying on cooperative self-organization \cite{GleizesEtAl1999}. 
% 
% 
% A popular paradigm for on-chip learning is self-organization. 
Local learning and adaptation mechanisms lead the neural network to self-organize and thereby implement a desired computation, for example with self-organized maps or plasticity rules in SNNs \cite{KhacefEtAl2019Self}. 
% As is common with multi-scale dynamics (Section \ref{ss:dimensions}), it may be undecidable which local rules yield a particular global behavior.
% Thus, programming with self-organization can be exploratory to investigate what behavior emerges from different local rules, or it can be goal-driven when local rules are optimized to satisfy some behavioral constraints.
% Self-organization can also take place directly in physics to grow computing devices where the device is not explicitly designed \cite{CucchiEtAl2021,TalsmaEtAl2020Synaptic,GrzybowskiEtAl2009,BoseEtAl2015}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NEUROMORPHIC PROGRAMMING CONCLUSION
%%%
%Most fall into three categories: 
%optimize SNN with supervised training
%%point tools for optimizing SNN parameters with supervised training, usually with deep learning techniques (SNN Conversion Toolbox [21], SLAYER [22], Whetstone [138], and EONS [139]), 
%low-level programming for SNNs
%%SNN simulators for conventional architectures that offer low-level programming APIs (Brian 2 [140], BindsNET [141])
%low-level interfaces and runtime frameworks for configuring neuromorphic hardware
%%(PyNN [142], Fugu [143], and our own NxSDK).
%How to move past that toward high-level programming abstractions for neuromorphic hardware?
%Exception: nengo
%%Nengo provides a good ﬁrst step toward a productive development framework, but a fundamental expansion of the abstractions and compositional tools will be needed to encompass the wider scope of computation that neuromorphic networks support, especially the stochastic, temporally coded, and directly trained networks that have demonstrated the greatest quantitative gains in latency and efﬁciency.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%design: % analogy to manual design -> starting point
%	neuromorphic circuit design
%	
%plasticity: % mostly manually designed (emergent programming)
%	local learning rules
%
%			 % leverage existing work in ANNs & SNNs (simulated)
%interfacing: % communication & interfacing aspect of programming
%	compile existing architecture 
%	convert ANN architecture to SNN 
%
%optimization: % training & automatic design
%	spiking backprop
%	reservoir computing
%	evolutionary (training and designing)
%
%compilation:
%	top-down with low-level instructions
%		language-like discrete operations
%		interface to implement NNs on different hardware 
%		does not move to higher-level behavioral descriptions
%	bottom-up and hierarchical with composable primitives
%		NEF
%		neurocomputational primitives (NSM, TDE, etc.)
%		spiking neural algorithms (SNA) with Fugu
%
%neuromorphic programming:
%	higher level of abstraction
%	need building blocks (primitives)

%%%%%%%%%%%%%%%%%%%%

% Summary: 
%cybernetics (signal processing, control engineering, dynamical systems),
%optimization and search (machine learning, evolution, probabilistic, inductive, synthesis),
%design (parallel, concurrent, dataflow, compilation),
%other (natural language, constraint),
%reservoir (cybernetics, optimization)
% Existing work for neuromorphic
%ML: spike-based plasticity, backprop, ANN transfer, reservoir computing, evolution,
%Neuromorphic compilation: Loihi, Tianjic
%Neuromorphic synthesis: Neftci
%{\color{red}Non-ML: graph algorithms, random walks (others? see Schuman2022 etc)}

% Other stuffs
%%%%%%%%%%%%%%%%%%%%%%%%%
%Differentiable self-organizing systems based on CAs
%@article{mordvintsev2020thread:,
%  author = {Mordvintsev, Alexander and Randazzo, Ettore and Niklasson, Eyvind and Levin, Michael and Greydanus, Sam},
%  title = {Thread: Differentiable Self-organizing Systems},
%  journal = {Distill},
%  year = {2020},
%  note = {https://distill.pub/2020/selforg},
%  doi = {10.23915/distill.00027}
%}

==> old/text-abstract-old.tex <==
% motivation - programming crucial, current methods lacking, future outlook promising
The value of neuromorphic computers depends crucially on our ability to program them for relevant tasks. Currently, neuromorphic computers are mostly limited to machine learning methods adapted from deep learning.
However, neuromorphic computers have potential far beyond deep learning if we can only make use of their computational properties to harness their full power. 
% claim: paradigm shift necessary
Neuromorphic programming will necessarily be different from conventional programming, requiring a paradigm shift in how we think about programming in general.
% contribution: 1) conceptual cleanup, 2) exploration of paradigms/approaches
The contributions of this paper are 1) a conceptual analysis of what `programming' means in the context of neuromorphic computers and 2) an exploration of existing programming paradigms that are promising yet overlooked in neuromorphic computing. 
% goal: expand horizon
The goal is to expand the horizon of neuromorphic programming methods, thereby allowing researchers to move beyond the shackles of current methods and explore novel directions.

%The value of neuromorphic computers depends crucially on our ability to program them for relevant tasks. Currently, neuromorphic computers are mostly limited to machine learning methods adapted from deep learning. However, neuromorphic computers have potential far beyond deep learning, if we can only make use of their computational properties to harness their full power. Neuromorphic programming will necessarily be different from conventional programming, requiring a paradigm shift in how we think about programming in general. The contributions of this paper are 1) a conceptual analysis of what `programming' means in the context of neuromorphic computers and 2) an exploration of existing programming paradigms that are promising yet overlooked in neuromorphic computing. The goal is to expand the horizon of neuromorphic programming methods, thereby allowing researchers to move beyond the shackles of current methods and explore novel directions.

%Based on existing work from computer and computational science, we explore what neuromorphic programming may look like and what paradigms may be promising, in order to expand the horizon of neuromorphic programming methods.
%, what sort of abstractions may be possible, 
%We embrace the diversity of programming paradigms that may be useful for neuromorphic computing. 
%The ﬁeld of neuromorphic computing is thriving, with many physical realizations at different levels of maturity. 
% configuration is more low-level than programming "programming without abstractions"

==> tikz-figure.tex <==
%\begin{tikzpicture}[node distance=1cm, auto,]
%	\node[punkt] (intent) {Intention};
%	\node[punkt, right=2cm of intent] (spec) {Specification}
%		edge[pil, <-] node[auto, above left] {} (intent);
%%	\node[punkt, below right=of intent] (idea) {Idea}
%%		edge[pil, <-, bend left=10] node[auto] {thinking} (intent);
%	\node[punkt, right=2cm of spec] (prog) {Program}
%%		edge[pil, <-, bend left=10] node[auto, below right=-0.2cm] {coding} (idea)
%		edge[pil, <-, red] node[auto, above right=-0.2cm] {} (spec);
%%		edge[pil, <-, dashed, gray] node[auto, above] {NLP} (intent);
%%	\draw[->] (prog) to[in=-30, out=-50, looseness=3.8] node[text=gray, midway, below] {compile} (prog);
%%	\draw[line width=0.75pt,dashed] (8,2) -- (8,-2); 
%
%
%%	\node[punkt, text width=5em, right=1cm of prog] (inp) {Input};
%%	\node[text width=6.5em,text centered,right=of inp] (mach) {Machine};	
%%	\node[text width=6.5em,text centered,below=0.2cm of mach] (conf) {Configuration};
%%	\node[draw,very thick,rounded corners,fit=(mach) (conf)] {};
%%	\draw[line width=0.75pt] (11,-0.35) -- (13.3,-0.35);
%%	\node[punkt, text width=5em, right=of mach] (out) {Output};
%%	\node[punkt, above=2.5em of mach] (env) {Environment};
%%	\draw [pil,->, shorten >= 4pt] (inp) -- node [name=in] {} (mach);
%%	\draw [pil,->, shorten <= 4pt] (mach) -- (out);
%%	\draw [pil,->, shorten >= 4pt] (out) |- (conf);
%%	\draw [pil,->, shorten >= 4pt] (in) |- (conf);
%%	\draw [pil,<->, shorten <= 4pt] (mach) -- (env);
%%%	\draw [pil,->, shorten >= 4pt] (prog) to[in=10] (conf);
%%	\node[rectangle,draw,very thick,dashed,minimum width = 8.5cm,minimum height = 3.6cm, anchor=north west] (rect) at (8,1.9) {};
%%	\draw [pil,->,shorten <= 4pt] (prog) -- (rect);
%\end{tikzpicture}
\begin{tikzpicture}[node distance=1cm, auto,]
	\node[punkt] (intent) {Intention};
	\node[punkt, above right=of intent] (spec) {Specification}
		edge[pil, <-, bend right=10] node[auto, above left] {formalization} (intent);
	\node[punkt, below right=of intent] (idea) {Idea}
		edge[pil, <-, bend left=10] node[auto] {thinking} (intent);
	\node[punkt, right=4cm of intent] (prog) {Program}
		edge[pil, <-, bend left=10] node[auto, below right=-0.2cm] {coding} (idea)
		edge[pil, <-, bend right=10] node[auto, above right=-0.2cm] {synthesis} (spec);
		edge[pil, <-, dashed, gray] node[auto, above] {NLP} (intent);
%	\draw[->] (prog) to[in=-30, out=-50, looseness=3.8] node[text=gray, midway, below] {compile} (prog);
%	\draw[line width=0.75pt,dashed] (8,2) -- (8,-2); 


	\node[punkt, text width=5em, right=1cm of prog] (inp) {Input};
	\node[text width=6.5em,text centered,right=of inp] (mach) {Machine};	
	\node[text width=6.5em,text centered,below=0.2cm of mach] (conf) {Configuration};
	\node[draw,very thick,rounded corners,fit=(mach) (conf)] {};
	\draw[line width=0.75pt] (11.4,-0.35) -- (13.5,-0.35);
	\node[punkt, text width=5em, right=of mach] (out) {Output};
	\node[punkt, above=2.5em of mach] (env) {Environment};
	\draw [pil,->, shorten >= 4pt] (inp) -- node [name=in] {} (mach);
	\draw [pil,->, shorten <= 4pt] (mach) -- (out);
	\draw [pil,->, shorten >= 4pt] (out) |- (conf);
	\draw [pil,->, shorten >= 4pt] (in) |- (conf);
	\draw [pil,<->, shorten <= 4pt] (mach) -- (env);
%	\draw [pil,->, shorten >= 4pt] (prog) to[in=10] (conf);
	\node[rectangle,draw,very thick,dashed,minimum width = 8.5cm,minimum height = 3.6cm, anchor=north west] (rect) at (8,1.9) {};
	\draw [pil,->,shorten <= 4pt] (prog) -- (rect);
\end{tikzpicture}
